Control Barrier Functions and Input-to-State Safety with Application to Automated Vehicles

Balancing safety and performance is one of the predominant challenges in modern control system design. Moreover, it is crucial to robustly ensure safety without inducing unnecessary conservativeness that degrades performance. In this work we present a constructive approach for safety-critical control synthesis via Control Barrier Functions (CBF). By filtering a hand-designed controller via a CBF, we are able to attain performant behavior while providing rigorous guarantees of safety. In the face of disturbances, robust safety and performance are simultaneously achieved through the notion of Input-to-State Safety (ISSf). We take a tutorial approach by developing the CBF-design methodology in parallel with an inverted pendulum example, making the challenges and sensitivities in the design process concrete. To establish the capability of the proposed approach, we consider the practical setting of safety-critical design via CBFs for a connected automated vehicle (CAV) in the form of a class-8 truck without a trailer. Through experimentation we see the impact of unmodeled disturbances in the truck's actuation system on the safety guarantees provided by CBFs. We characterize these disturbances and using ISSf, produce a robust controller that achieves safety without conceding performance. We evaluate our design both in simulation, and for the first time on an automotive system, experimentally.

==> _Aux/old_text.tex <==
%We consider an automated truck with the drive-by-wire technology that provides active control over the longitudinal motion.
%, we have the following mechanical model that describes the longitudinal motion of the truck:
%\begin{equation}
%    \dot{v} = {\rm sat} (u) + d(t),
%\end{equation}
%where $v$ is the longitudinal velocity. The input $u$ is the desired longitudinal acceleration with simplifications in power generation and transmission along with time delays in sensing, computing and communication are lumped as an input disturbance $d:\R_{\geq0}\to\R$. The input is bounded with the saturation function due to physical limitations on tires and the engine:
%\begin{equation}
%    \label{eq:truck_aBar}
%    u \in [-\underline{a}, \overline{a}].
%\end{equation}
%Consider the following car following problem with a preceding vehicle:
%\begin{equation}   \label{eq:truck_model}
%    \begin{split}
%        \dot{D} &=v_{\rm L}-v, \\
%        \dot{v} &={\rm sat}(u)+d(t), \\
%        \dot{v}_{\rm L} &= a_{\rm L},
%    \end{split}
%\end{equation}
%where $D$ is the bumper-to-bumper headway distance between vehicles, $v_{\rm L}$ and $a_{\rm L}$ are longitudinal velocity and acceleration of the preceding vehicle with $a_{\rm L}$ bounded as
%\begin{equation}
%    \label{eq:truck_aLBar}
%    a_{\rm L} \in [-\underline{a}_{\rm L}, \overline{a}_{\rm L}].
%\end{equation}
%Also, we have
%\begin{equation} \label{eq:truck_speedlimit}
%    v,v_{\rm L} \in [0,\overline{v}].
%\end{equation}

%\begin{table}[t]
%\small
%\centering {
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
%\hline
% $\mb{\underline{a}}$ &  $\mb{\underline{a}_{\rm L}}$ & $\mb{\overline{v}}$  & $\mb{D_{\rm sf}}$ & ${\boldsymbol\theta}$ & ${\boldsymbol\eta}$  & ${\boldsymbol \xi}$   & ${\boldsymbol\zeta}$  & ${\boldsymbol\omega}$ \\ \hline
% 6 & 10 & 20 & 2   & 1.1   & 0.62 & 0.03 & -0.03 & -0.03 \\ 
% $[\frac{\rm m}{\rm s^2}]$  &  $[\frac{\rm m}{\rm s^2}]$ &  $[\frac{\rm m}{\rm s}]$  &   ${\rm [m]}$ &   ${\rm [s]}$ &    ${\rm [s]}$ &     $[\frac{\rm s^2}{\rm m}]$  &  $[\frac{\rm s^2}{\rm m}]$    &   $[\frac{\rm s^2}{\rm m}]$    \\ \hline
%\end{tabular}
%}
%\caption{Parameters corresponding to the car following problem and $\hat{h}(\mb{x})$ defined in \eqref{eq:truck_CDF}.}
%\label{tab:parameters}
%\end{table}
%\begin{figure}[!t]
%	\centering
%	\includegraphics[width=\linewidth]{Figures/Fig20.eps}\\
%	\caption{\small (a) Saturation function and (b) range policy \eqref{eq:truck_V}}  \label{Fig:carfollowing}
%\end{figure}

